Stochastic Gravitational-Wave Background from Stellar Core-Collapse Events

We estimate the stochastic gravitational-wave background arising from all stellar core-collapse events in the universe based on the gravitational-wave signal predictions of recent numerical simulations. We focus on waveforms from slowly or non-rotating stars and include rapidly rotating, highly massive progenitors as extreme case limits. Our most realistic estimates are more than one hundred times below the sensitivity of third-generation terrestrial gravitational-wave detectors and likely weaker than cosmological contributions to the stochastic gravitational-wave background.

==> dedf.tex <==
The spectral energy density of the GWs emitted by a core-collapse supernova is 
required in order to calculate its contribution to \omgw. The energy radiated as GWs to infinity by
a source is given by \citep{gravity}
\begin{equation}
    \egw = \int_{0}^{t} \mathrm{d}\tau \int T_{0\nu} n^{\nu} r^2 \mathrm{d}\Omega,
\end{equation}
where the angular integral should be performed over a spherical shell at infinity that enclose the source.
The vector $n^{n}$ is a spacelike unit vector perpendicular the surface of the spherical shell, $r$ denotes
the radius of spherical coordinate system, and $T_{\mu\nu}$ denotes the GW energy-momentum tensor which,
in the transverse-traceless (TT) gauge, is given by
\begin{equation}
    T_{\mu\nu} = \langle (\partial_\mu h_{\gamma\lambda}^{\mathrm{TT}})(\partial_\nu h^{\gamma\lambda}_{\mathrm{TT}}) \rangle
\end{equation}
